A physics-informed, vision-based method to reconstruct all deformation modes in slender bodies

This paper is concerned with the problem of estimating (interpolating and smoothing) the shape (pose and the six modes of deformation) of a slender flexible body from multiple camera measurements. This problem is important in both biology, where slender, soft, and elastic structures are ubiquitously encountered across species, and in engineering, particularly in the area of soft robotics. The proposed mathematical formulation for shape estimation is physics-informed, based on the use of the special Cosserat rod theory whose equations encode slender body mechanics in the presence of bending, shearing, twisting and stretching. The approach is used to derive numerical algorithms which are experimentally demonstrated for fiber reinforced and cable-driven soft robot arms. These experimental demonstrations show that the methodology is accurate (<5 mm error, three times less than the arm diameter) and robust to noise and uncertainties.

==> 02_Cover.tex <==
Dear Editor,

we are please to submit our paper "A physics-informed, vision-based method to reconstruct all deformation modes in slender bodies" for consideration to RA-L with ICRA.

In this paper we introduce a novel, robust and accurate physics-informed approach, based on Cosserat rod theory, to reconstruct from camera images shape and all six strain functions (normal and binormal bending and shear, twist and stretch) of a slender elastic body. This problem is of relevance in biology and engineering alike, to gain insight into compliance-mediated principles of control. Further, our methodology is experimentally demonstrated for fiber reinforced and cable-driven soft robot arms. These  demonstrations show that the approach is accurate (<5 mm error, three times less than the arm diameter) and robust to noise and uncertainties.

We believe this work ought to be of interest to roboticists, biologists, physicists and control experts. Hence, our submission to RA-L with ICRA.

Sincerely

Mattia Gazzola


==> 05_Todo_List.tex <==
\clearpage

\newcommand{\answerYes}[1][]{\textcolor{blue}{[Yes] #1}}
\newcommand{\answerNo}[1][]{\textcolor{orange}{[No] #1}}
\newcommand{\answerNA}[1][]{\textcolor{gray}{[N/A] #1}}
\newcommand{\answerTODO}[1][]{\textcolor{red}{\bf [TODO]}}

\section*{Checklist}
%Please read the instructions below carefully and follow them faithfully.

%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerNA{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
	\item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Naveen's code}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}
\end{enumerate}

==> 06_Unused.tex <==
% =========== Introduction =============================== 
% %% Motivation on studying CSA
% Soft Continuum Arms \cite{Xie2018,Shen2017,Huang2019,Zhang2019,Wang2017,Bern2019,Uppalapati2018} have demonstrated the capability of performing complex and dexterous maneuvers similar to ubiquitous slender objects in nature and biology.
% %For example, octopus has been shown to exploit rich shaping and functionality of the soft-arm to find the solution to the provided tasks \cite{TODO}.
% Current SCA utilize the inherent compliance and adaptability of the soft materials and have been successfully deployed in several applications like surgery \cite{Lloyd2021,Wang2017}, agriculture \cite{Chowdhary2019, Uppalapati2020a,Tapia2020,VanHenten2002}, and assistive devices\cite{Ansari}.
% In order to develop a robust framework for design, modeling/simulation and control, accurate characterization of shape and deformation of the SCA is of paramount importance.
% %Many existing SCA designs harvest properties of the soft material, such as compliance and adaptability, in the application such as medical surgery \cite{Lloyd2021,Wang2017}, agriculture \cite{Chowdhary2019,Tapia2020,VanHenten2002}, and assistive devices \cite{Ansari} etc. % agriculture, medical surgery, 
% %search and rescue \cite{Galloway2016}
% %millitary \cite{Grissom2006}
% %factory production line\cite{Yamanaka2020}
% %Since problem solving using the SCA involves manipulating an elastic behavior, accurate characterization of shape and deformation is the first step to develop robust frameworks for — design, modeling/simulation, control, and application.

% Current sensing methods for the SCA are either invasive or expensive.
% Invasive methods such as EGaIn sensor \cite{Cho2021,Morrow2016,Park2013} on a SCA effects the physics and the performance of the SCA.
% Furthermore, invasive sensors could be fabrication intensive and should be considered apriori during the design of the SCA. Shape sensing of the 
% SCA can also be done by placing several magnetic sensors along the length of the SCA \cite{Bergamini2014}. The magnetic sensors detect the pose and this information is used for accurate posture reconstruction. However, the use of several magnetic sensors makes the sensing system expensive.
% Hence, we adopt a multi-vision tracking mechanism \cite{Gong2018} \cite{reilink2013} to minimize the physical interference and also have a cost-effective solution.

% Vision-based methods are effective reconstructing shape and motion of an object from camera images, and multiple cameras overcome occlusion and aperture issues \cite{Gong2018}.
% Several existing vision algorithms serves purpose of recognizing the trajectory of the slender body, such as clustering \cite{Reiter2011}, skeletonization \cite{Fan2020,Inoue2021}, and deep learning \cite{Mathis2018}.
% Even though these methods are easy to implement and practical, limitation often comes in quantifying the body rotations and handling scenarios when some regions are occluded.
% In this paper, in order to obtain the entire posture of the SCA we propose a vision-based method that can directly evaluate the 3D position and orientation at any desired cross-section of the arm.
% %The other studies attempts to reconstruct deformation using point-cloud data given by depth camera \cite{Camarillo2008}, and extended algorithm, called Self-Organized Maps \cite{Xu2018} \cite{Croom2010}, establish continuous information using the unsupervised neural-network.

% %% Limitation/Comparison to previous reconstruction work - challenges in reconstruction and modeling
% We use a multi camera system to capture several discrete points along the length of the SCA. 
% Several methods have been proposed to use this discrete points and orientation information to obtain continuous strain information of the SCA.
% %Once the discrete points and orientation are captured by the tracking, several studies have been done to reconstruct the arm into a continuous strain information.
% %The imminent problem of the reconstruction arrives from the intrinsic non-linearity of the continuum arm.
% Fan \textit{et al}.\cite{Fan2020} and Albeladi \textit{et. al} \cite{AlBeladi2020} used basis functions to fit the shape of the SCA. However, fitting and interpolation methods are limited in capturing the extension, twist, and shear of the body.
% Although machine learning reconstruction \cite{Scharff2021,Reiter2011} and gradient-based reconstruction \cite{Manakov2021} methods have improved the accuracy and are widely available, they do not utilize the physics of the soft-arm models.
% A closely related work done by Fu \textit{et. al} \cite{Fu2021} utilize the special Cosserat rod model to derive all modes of strain given the set of reference position and orientation data. 
% However, the optimization was performed in a piecewise fashion that resulted in discontinuity in the computed strains. In this work, we are interested in building a physics-based method that has smooth strains and thus reconstructs the final pose/configuration of the SCA.

% %% Contribution
% In this paper, we propose a multi-camera system to directly evaluate the shape of the arm in 3D-space.
% In addition, we introduce a novel smoothing method to reconstruct continuous position and orientation information that conforms to the special Cosserat rod model.
% We demonstrate our tracking and reconstruction method on FREE \cite{Bishop-moser2015} based SCA and a cable-driven arm \cite{Bern2019}.
% The proposed smoothing method computes a reasonable reconstruction with smoothed strain functions on all 6 degree of freedoms.
% We emphasize that the experiment and the reconstruction method are generally applicable to any flexible soft actuators.
% We provide Python code and example dataset for our method.
% %Lastly, we evaluate the accuracy and robustness.

% % (Optional) Outline of the paper


% =============== Fabrication Panel Caption =========================== 
% Fabrication Panel Caption
% (Right) Soft-arm fabrication process. 
% %We apply cement on a rubber tube and wrap fiber with specified angles throughout the tube to constrain motion.
% An adhesive cement is applied on an elastic tube to adhere constraining fiber.
% The guide rail and the stepper motor are used to maintain a consistent pitch and an angle of the fiber.
% After the cement dries, a desire length of a segment is trimmed.
% Lastly, multiple FREEs can be assembled in parallel and/or serial using 3d printed connectors.
%We attach markers on BR2 and connect to compressed air source with pneumatic valves.
%The valves are connect to a rasberry-pi, which can be controlled real-time with a computer.
%We place BR2 in the center of a frame with five cameras surrounded.

% ================ Calibration and Camera Setup ========================== 
% We prepared an apparatus, shown in the Fig.\ref{fig:1}, to mount a soft-arm at the center surrounded by five cameras (AKASO EK7000, 60-fps, 1080p).
% The aluminum profile allows relocating the camera strategically, such that all tracking points are visible at least by two camera throughout the complex motions.
% Each camera is associated with 11 parameters $\{L_1, L_2, L_3, ..., L_{11}\}$ \cite{TODO}
% that relates the mapping between the lab frame with physical distances to the reference frame with pixels.
% Parameters changes upon the bearing and the position of each camera, and parameters are estimated during the calibration process.

% \textbf{The Direct Linear Transformation (DLT)} \cite{TODO} process multiple 2D images to approximate the 3D coordinate described by the following 
%     \begin{align}
%         u &= \frac{L_1x+L_2y+L_3z+L_4}{L_9x+L_{10}y+L_{11}z+1} \\
%         v &= \frac{L_5x+L_6y+L_7z+L_8}{L_9x+L_{10}y+L_{11}z+1}
%     \end{align}
%     \begin{align}
%         \begin{bmatrix}uL_9-L_1 & uL_{10}-L_2 & uL_{11}-L_3 \\ vL_9-L_5 & vL_{10}-L_6 & vL_{11}-L_7 \\ & \vdots & \end{bmatrix}
%         \begin{bmatrix}x \\ y \\ z\end{bmatrix} = 
%         \begin{bmatrix}L_4-u \\ L_8-v \\ \vdots \end{bmatrix}\label{eq:DLT}
%     \end{align}.
% We note that once the camera parameters are determined, the method provides bidirectional mapping allowing overlap of the processed data on the video.
%not clear to me how overlap relates to bidirectional mapping

% \textbf{Camera Calibration} must be done thoroughly to achieve reliable accuracy with DLT method.
% While the checkerboard patterns is a common calibration reference \cite{TODO}, we noticed the planar calibration causes extrapolation of the out-of-plane motion.
% To capture as many reference points that enclose workspace, we developed our own calibration tool as shown in Fig.\ref{fig:2}.
% The equispaced flags are hanging on the rod to provide the calibration and yz-plane, and the slide rail allows to move the plane to multiple x-positions.
% In an attempt to automate the calibration, a DLT method, which requires minimum 6 points, is regularly used to predict the remaining references, and Harry's corner detection algorithm \cite{TODO} corrected the predicted points to be located at the tip of the flag.
% In result, more than 1000 points could be collected that is simultaneously visible by all cameras over the volume of our workspace.
% % The distortion correction \cite{Wang1992} is first applied to correct the wide-view lens distortion, and the camera parameters $L$ are determined by 
% % \begin{align}
% %     %\begin{bmatrix}x & y & z & 1 & 0 & 0 & 0 & 0 & -ux & -uy & -uz \\ 0 & 0 & 0 & 0 & x & y & z & 1 & -vx & -vy & -vz  \\ \vdots \end{bmatrix}
% %     %\begin{bmatrix}L_1 \\ L_2 \\ \vdots \\ L_{11} \end{bmatrix} = 
% %     %\begin{bmatrix}u \\ v \\ \vdots \end{bmatrix}
% %     \begin{bmatrix}x & y & z & 1 & -ux & -uy & -uz \\ & \vdots & \end{bmatrix}
% %     \begin{bmatrix}L_1 \\ L_2 \\ \vdots \\ L_{11} \end{bmatrix} = 
% %     \begin{bmatrix}u \\ \vdots \end{bmatrix} \\
% %     \begin{bmatrix} x & y & z & 1 & -vx & -vy & -vz  \\ \vdots \end{bmatrix}
% %     \begin{bmatrix}L_5 \\ L_6 \\ \vdots \\ L_{11} \end{bmatrix} = 
% %     \begin{bmatrix} v \\ \vdots \end{bmatrix}
% % \end{align}.
% Given the amount redundancy of the system, such as multiple camera and densely populated points, we consistently achieved the calibration error at most $5\pm 4$ pixels, which correspond to the reprojection error of $1.4 \pm 1.2 mm$ throughout the workspace.
% %The camera calibration step is done at the end of the each experiment to ensure any deviation in camera parameters in-between the experiment.
% %In practice, the motion can be captured with workable amount of precision if the motion is captured within the DLT calibration space, which reduces the possibility of extrapolation.
% %The re-projection error provides rough measurement the accuracy of our DLT mapping in image space and lab space.
% %The calibration error is measured using the re-projection errors, which characterize the difference between mapping coordinate versus true coordinate using the calibration points.
% %Due to the influence of lens distortion and noises,
% For each camera recordings, we manually select the initial reference markers on the arm, and the Lucas-Kanade's optical flow method \cite{TODO} is used to trace the markers throughout the video.
% The algorithm assumes the intensity of the object remains relatively constant in spatiotemporal domain
% \begin{align}
%     I(\vec{x},t) &= I(\vec{x}+\vec{u},t+1) \\
%     \nabla I \cdot \vec{u}+I_t&=0 \label{eqn:OF}
% \end{align}
% where $I(\vec{x},t)$ represent the intensity of the image at the image position $\vec{x}=(x_1, x_2)$ and time $t$.
% To solve for two velocity component $\vec{u}=(u_1, u_2)$, we select the window of pixels to over-determine the system of equations \eqref{eqn:OF}.
% %In order to enhance the automated data processing, sharp contrasts in the background were covered with white cloth and papers. % this sentence and the next sentence kinda break the flow about velocity. Can we put them after cv2?
% In practice, the window of size $19\times 19$ is used to capture the size of the marker.
% In addition, the velocity is first computed in the lower resolution representation to detect high-velocity and blurred markers, and the method can be repeated in multi-layer fashion called pyramid method \cite{TODO}.
% The implementation used CV2(OpenCV) library.

% \textbf{Occlusion Handling}
% One major challenge in vision-based tracking system comes in occlusion handling, since the marker on the arm frequently disappears and reappears from the camera view.
% The disappearance can be handled by monitoring the confidence of optical flow, which typically measured by the eigenvalues.
% The equation \eqref{eqn:OF} with multiple pixel can be represented as
% \begin{align}
%     \begin{bmatrix}
%     I_x^1 & I_y^1 \\ 
%     I_x^2 & I_y^2 \\ 
%     \vdots &
%     \end{bmatrix}
%     \begin{bmatrix}
%     u_1 \\ u_2
%     \end{bmatrix}
%     &= -
%     \begin{bmatrix}
%     I_t^1\\ 
%     I_t^2\\ 
%     \vdots 
%     \end{bmatrix} \\
%     \textbf{A}\vec{u} &= \textbf{b} \\
%     \textbf{A}^\transpose \textbf{A} &= \begin{bmatrix}
%     \sum I_x^2 & \sum I_xI_y \\
%     \sum I_xI_y & \sum I_y^2
%     \end{bmatrix}\label{eqn:OF_matrix}
% \end{align}
% which implies the conditioning of the matrix $\textbf{A}^\transpose\textbf{A}$ determines the well-posedness of the optical flow algorithm.
% If one of the eigenvalue of the matrix \eqref{eqn:OF_matrix} is too small, which occurs when the contrast gradient $\nabla \vec{u}$ in one direction is significantly greater than any other direction, the case is called ill-conditioned aperture problem.
% Such case is the indication of a point placed on the horizon, and we set a threshold $\min(\lambda_1, \lambda_2)<\gamma$ to determine whether point disappeared.

% Handling reappearance requires more sophisticated algorithm, because the appearance of the marker cannot be determined by a single camera. With assist of pattern recognition algorithm, an entire image can be searched to detect the reappearance of markers, but methods are often prone to false positive.
% Instead, we utilize the inverse DLT mapping.
% If the 3D coordinate of a particular marker position is known, an inverse DLT predicts where the marker should appears.
% Using this estimation, we can compare the color and intensity spectrum of the marker, measured by other visible cameras, to determine whether the marker is still occluded.

% ========== Problem Formulation ===================

% \section{Problem Formulation}
% In this paper, a novel ideal on soft arm smoothing reconstruction is proposed. By using techniques in optimization, a smooth curve that captures all six modes of strains is reconstructed based on the provided noisy data measurements $\dataset$. In the following subsections, the models of the special Cosserat rod theory and the data collection are firstly presented, the physical meaning of the decision variable $\decisionvariables$ is then introduced and the objective function $\cost$ together with the proper optimization problem statement are lastly proposed. In general, the optimization problem for smoothing reconstruction has the following form:
% \begin{subequations}\label{eq:general_smoothing_problem}
% 	\begin{align}
% 		\min_{\decisionvariables(\cdot)}&\quad\text{objective function (energy + error cost)}\\
% 		\text{subject to}&\quad \text{kinematics of a Cosserat rod}\\
% 		&\quad \decisionvariables\text{-related constraints}
% 	\end{align}
% \end{subequations}

% \textbf{Data Collection and the Cosserat Rod Model of a Soft Arm}
% The experiment setup is shown in the figure \ref{fig:1}. A soft arm with length $L$ is fixed at the base and it is parameterized by the arc-length parameter $s\in[0,L]$ with $s=0$ as the base and $s=L$ as the tip. The pose of the arm  at each cross-section $s$ (with respect to the fixed lab frame $\set{\mathrm{e}_1, \mathrm{e}_2, \mathrm{e}_3}$ at the base) is represented by an element $\pose(s)$ in the special Euclidean group, i.e. 
% \begin{equation}
%     \pose(s)=\begin{bmatrix}\orientation(s)&\positions(s)\\0&1\end{bmatrix}\in\SE{3}
% \end{equation}
% where the directors $\orientation(s)\in\SO{3}$ and the positions $\positions(s)\in\reals^3$. Along the soft arm, $N_\data$ number of colored markers are placed with known locations. Their locations and noisy pose measurements are denoted as a data set $\dataset=\set{s_j,\pose_j}_{j=1}^{N_\data}$. (Detail marker pose measurement is shown in Sec. \ref{sec:Experimental_Setup}) In this paper, a soft arm is modeled as a special Cosserat rod which means that its pose should follow the kinematic constraint
% \begin{subequations}\label{eq:kinematics}
%     \begin{equation}
%         \tfrac{\partial}{\partial s}\pose(s)=\pose(s)\twists(s),\quad\pose(0)=\pose_0
%     \end{equation}
%     where $\pose_0$ is given and $\twists(s)\in\mathfrak{se}(3)$ is parameterized by strains $\strains(s)$ in the following form
%     \begin{equation}
%         \twists(s)=
%         \begin{bmatrix}
%             [\curvatures]^\times&\shears\\
%             0&0
%         \end{bmatrix},\quad
%         \strains(s)=\begin{bmatrix}\curvatures(s)\\\shears(s)\end{bmatrix}
%     \end{equation}
%     with bending strains $\curvature_1(s),\curvatures_2(s)\in\reals$, twisting strain $\curvature_3(s)\in\reals$, shearing strains $\shear_1(s),\shear_2(s)\in\reals$, stretching strain $\shear_3(s)\in\reals^+$ and $[\cdot]^\times$ as an isomorphic map from $\reals^3$ to $\mathfrak{so}(3)$:
%     \begin{equation*}
%         \begin{bmatrix}\curvature_1\\\curvature_2\\\curvature_3\end{bmatrix}^\times\defined
%         \begin{bmatrix}
%             0&-\curvature_3&~~\curvature_2\\
%             ~~\curvature_3&0&-\curvature_1\\
%             -\curvature_2&~~\curvature_1&0
%         \end{bmatrix}
%     \end{equation*}
% \end{subequations}

% The potential energy of a soft arm is then given by
% \begin{subequations}
%     \begin{equation}
%         \potential=\int_0^L \storedenergy(s,\strains(s))~\dif s
%     \end{equation}
%     where $\storedenergy:[0,L]\times\reals^6\to\reals$ is called the stored energy function. Here, we adopt a quadratic model
%     \begin{equation}
%         \storedenergy(s,\strains)=\tfrac{1}{2}\abs{\strains-\strains^\intrinsic}_\rigidity^2
%     \end{equation}
%     where $\rigidity(s)\in\reals^{6\times6}$ is the rigidity matrix, $\strains^\intrinsic(s)$ is the intrinsic strain and the weighted norm is defined as $\abs{x}_{\Matrix{R}}\defined\sqrt{\Vector{x}^\transpose\Matrix{R}\Vector{x}}$ for any vector $\Vector{x}\in\reals^\n$ and any positive definite matrix $\Matrix{R}\in\reals^{\n\times\n}$. 
% \end{subequations}

% \textbf{Decision Variable and its Physical Meaning}
% For given functions of strains $\strains$, one can integrate \eqref{eq:kinematics} to obtain the posture of a soft arm. It is natural to consider $\strains$ as the decision variables $\decisionvariables$. However, results of this setting give discontinuous strain solutions which is not physically feasible. \cite{Fu2021} Thus, we consider the rate of strains as the decision variables, i.e.
% \begin{equation}
%     \tfrac{\partial}{\partial s}\strains(s)=\decisionvariables(s),\quad \strains(0)=\strains_0
% \end{equation}
% where $\decisionvariables(s)\in\reals^6$ and $\strains_0$ given. This not only gives us a globally feasible solution but also avoid discontinuity in the strain functions.

% \textbf{Objective Function and Problem Statement}
% The last thing remained to be shown is the objective function which is taken to be in the form of
% \begin{subequations}\label{eq:cost_function}
%     \begin{equation}
%         \cost(\decisionvariables;\dataset)=\potential+\tfrac{\chi_\decisionvariables}{2}\norm{\decisionvariables}_{\mathcal{L}_2}^2+\sum_{j=1}^{N_\data}\Phi(\pose(s_j);\pose_j)
%     \end{equation}
%     where $\chi_\decisionvariables\geq0$ is the regularization coefficient, the $\mathcal{L}_2$-norm is defined as $\norm{\Vector{u}}_{\mathcal{L}_2}=(\int_0^L\abs{\Vector{u}(s)}^2\dif s)^{1/2}$ for any vector-valued function $u:[0,L]\to\reals^\n$, and the fit cost function $\Phi$ is defined as
%     \begin{equation}
%         \Phi(\pose(s_j);\pose_j)=\tfrac{\chi_\orientation}{2}\norm{\orientation(s_j)-\orientation_j}_\Frobenius^2+\tfrac{\chi_\positions}{2}\abs{\positions(s_j)-\positions_j}^2
%     \end{equation}
%     with $\chi_\orientation,\chi_\positions\geq0$ as regularization parameters and the matrix norm $\norm{\Matrix{X}}_\Frobenius\defined\sqrt{\displaystyle\Trace{\Matrix{X}^\transpose\Matrix{X}}}$ for any square matrix $\Matrix{X}\in\reals^{\n\times\n}$.
% \end{subequations}

% The first term of the cost function is the potential energy. It is assumed that the experiment is operated in a quasi-static mode, at each time frame the soft arm is at its stable equilibrium which means it is at its lowest possible potential energy. \cite{Fu2021,chang2020energy} The second term is the regularization of the decision variable which is the same as regularization on the strain rate. This comes up naturally since the sudden rate change in strains is not common in the soft arm. This regularization term also serves as the characterization of the unknown forces and couples applied to the system. In the case of high distributed load, higher strain rates are allowed and thus a lower regularization coefficient $\chi_\decisionvariables$ is chosen and vice versa. The last term is the summation of the reconstruction fit costs $\Phi$. \cite{AlBeladi2020} The values of the coefficients in the fit cost function ($\chi_\orientation$ and $\chi_\positions$) depend on how accurate of the data set $\dataset$ is provided. If the information in the data is highly accurate, the higher values of the coefficients are chosen.

% Finally, an optimization problem for the reconstruction of a posture $\pose$ with smooth strains $\strains$ is then properly proposed in the following form
% \begin{subequations}
% 	\begin{align}
% 		\min_{\decisionvariables(\cdot)}&\quad\cost(\decisionvariables;\dataset)\\
% 		\text{subject to}&\quad \tfrac{\partial\pose}{\partial s}=\pose\twists,\quad\pose(0)=\pose_0\label{eq:pose_evolution}\\
% 		&\quad \tfrac{\partial\strains}{\partial s}=\decisionvariables,\quad\strains(0)=\strains_0\label{eq:strains_evolution}
% 	\end{align}
% \end{subequations}
% where $\cost$ takes the form of \eqref{eq:cost_function}, $\pose_0$ and $\strains_0$ are given and the decision variable $\decisionvariables\in\mathcal{U}=\set{u(s)\in\reals^6:s\in[0,L]}$.



% =============== Method =========================== 
% \section{Solution: Arm Reconstruction}
% In this section, a proposition of the necessary conditions of the solutions to the optimization problem \eqref{eq:smoothing_problem} is proposed. An iterative algorithm (forward-backward algorithm \cite{chang2020energy, chang2021controlling}) is then introduced based on the equations in the necessary conditions.

% \subsection{Necessary Conditions} % (HS)
% Solutions to \eqref{eq:smoothing_problem} should satisfy the Pontryagin's Maximum Principle with jump conditions.
% To write the proposition for the necessary condition, we first define the control Hamiltonian as
% \begin{equation}
% \begin{aligned}
% 	\staticHamiltonian(s,\pose, \strains,& \costatepose,\costatestrains,\decisionvariables)\\&=\inner{\costatepose}{\pose\twists}+\inner{\costatestrains}{\decisionvariables}-\storedenergy(s,\strains)-\tfrac{\chi_\decisionvariables}{2}\abs{\decisionvariables}^2
% \end{aligned}
% \end{equation}
% where $\costatepose(s)\in\reals^{4\times4}$ is the costate of $\pose(s)$ and $\costatestrains(s)\in\reals^6$ is the costate of strains $\strains(s)$.
% The inner product of any two vectors $\Vector{a},\Vector{b}\in\reals^{\n}$ is defined as $\inner{\Vector{a}}{\Vector{b}}\defined\Vector{a}^\transpose\Vector{b}$.
% The inner product of any two square matrices $\Matrix{A},\Matrix{B}\in\reals^{\n\times\n}$ is defined as $\inner{\Matrix{A}}{\Matrix{B}}\defined\Trace{\Matrix{A}^\transpose\Matrix{B}}$.
% Now we are ready to state the proposition.

% \begin{proposition} \label{prop:smoothing_problem_solution}
% 	Consider problem \eqref{eq:smoothing_problem}, any minimizer denoted by $\decisionvariables(s)$ with the corresponding state $(\pose(s),\strains(s))$ and costate $(\costatepose(s),\costatestrains(s))$ trajectories must satisfy the following necessary conditions including state evolution: \eqref{eq:pose_evolution} and \eqref{eq:strains_evolution}, reduced costate $(\internalcouples(s)\in\reals^3,\internalforces(s)\in\reals^3,\costatestrains(s)\in\reals^6)$ evolution:
% 	\begin{subequations}\label{eq:smoothing_problem_reduced_costate_evolution}
% 		\begin{align}
% 			\frac{\partial}{\partial s}\begin{bmatrix}\internalcouples\\\internalforces\end{bmatrix}&=-\begin{bmatrix}\curvatures\times\internalcouples+\shears\times\internalforces\\
% 			\curvatures\times\internalforces
% 		\end{bmatrix}\\
% 			\frac{\partial\costatestrains}{\partial s}&=-\begin{bmatrix}\internalcouples\\\internalforces\end{bmatrix}+\rigidity\left(\strains-\strains^\intrinsic\right) \label{eq:smoothing_problem_reduced_costatestrains_evolution}
% 	\end{align}
% \end{subequations}	
% 	with reduced jump condition:
% 	\begin{subequations}\label{eq:smoothing_problem_reduced_costate_jump_condition}
% 		\begin{align}
% 			\internalcouples(s_j^+)-\internalcouples(s_j^-)&=\chi_\orientation{\normalfont\text{vec}}\left[\orientation^\transpose\orientation_j-\orientation_j^\transpose\orientation\right]_{s=s_j}\\
% 			\internalforces(s_j^+)-\internalforces(s_j^-)&=\chi_\positions\left.\orientation^\transpose\left(\positions-\positions_j\right)\right|_{s=s_j}
% 		\end{align}
% \end{subequations}
% 	where the reduced costate $(\internalcouples(s),\internalforces(s))$ and the costate $\costatepose(s)$ have the following relation:
% 	\begin{subequations}\label{eq:costate_form}
% 		\begin{equation}
% 			\costatepose=\begin{bmatrix}
% 				\tfrac{1}{2}\orientation\left([\internalcouples]_\times+\symmetricpart\right)&\orientation\internalforces\\
% 				0&0
% 			\end{bmatrix}
% 		\end{equation}
% 		with the symmetric matrix $\symmetricpart$ written as
% 		\begin{equation}\label{eq:symmetricpart_form}
% 			\symmetricpart=-\orientation^\transpose\left[\left(\orientation\internalforces\right)\positions^\transpose+\positions\left(\orientation\internalforces\right)^\transpose\right]\orientation
% 		\end{equation}
% 	\end{subequations}
% 	and lastly, the pointwise maximization of control Hamiltonian which gives the zero gradient of $\staticHamiltonian$ with respect to $\decisionvariables$:
% 	\begin{equation}\label{eq:smoothing_problem_maxHamiltonian}
% 		\gradient_{\decisionvariables}\staticHamiltonian=\costatestrains-\chi_\decisionvariables\decisionvariables=0
% 	\end{equation}
% \end{proposition}	
% The proof of this proposition is mostly shown in {\color{red}the 3D energy shaping paper, but not sure how to cite it.} and the reduced jump condition \eqref{eq:smoothing_problem_reduced_costate_jump_condition} is shown by first calculating the jump condition
% \begin{subequations}\label{eq:smoothing_problem_costate_jump_condition}
% 	\begin{align}
% 		\costatepose(s_j^+)-\costatepose(s_j^-)&=\left.\gradient_\pose\Phi(\pose;\pose_j)\right|_{s=s_j}\label{eq:smoothing_problem_posturecostate_jump_condition}\\
% 		\costatestrains(s_j^+)-\costatestrains(s_j^-)&=\left.\gradient_\strains\Phi(\pose;\pose_j)\right|_{s=s_j}=0
% 	\end{align}
% \end{subequations}
% and secondly comparing terms using the relation in \eqref{eq:costate_form}.
% This proposition leads to a result of smooth strains, i.e. $\strains\in\continuous^1$.
% By utilizing these necessary conditions, we can use the forward-backward algorithm \cite{chang2021controlling,chang2020energy} to solve the optimization problem \eqref{eq:smoothing_problem}.

%\subsection{Brief Comparison} % (HS)
%Cosserat rods based reconstruction models \cite{AlBeladi2020,Fu2021} have aroused in recent years and the accurate strains estimation have always been a challenge. 

% \subsection{Algorithm}
% For a given data set $\dataset$, we use an iterative algorithm (forward-backward algorithm, see also Sec. III-C in \cite{chang2020energy}) to solve the optimization problem. At each iteration $k$, state trajectory ($\pose^{(k)}(s), \strains^{(k)}(s)$) is integrated forwardly from the base to the tip; reduced costate trajectory ($\internalcouples^{(k)}(s), \internalforces^{(k)}(s), \costatestrains^{(k)}(s)$) is then integrated backward from tip to base with jump condition at each $s=s_j$ where the data is provided; lastly, a gradient ascent method is used to update the optimal decision variable
% \begin{equation}\label{eq:update_law}
%     \decisionvariables^{(k+1)} = \decisionvariables^{(k)} + \alpha\gradient_\decisionvariables\staticHamiltonian^{(k)}
% \end{equation}
% where $\alpha>0$ is the update step size. Convergence results typically require sufficiently small values of the update step size. A brief pseudo code of the algorithm is presented in Algorithm \ref{alg:forward_backward}. A more comprehensive discussion on algorithms for solving this problem appears in \cite{chang2020energy}. 

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \begin{algorithm}[t]
% 	\caption{Solving the optimization problem \eqref{eq:smoothing_problem}}
% 	\label{alg:forward_backward}
% 	\begin{algorithmic}[1]
% 		\Require Data set $\dataset$ and state at base: $\pose(0)=\pose_0,~\strains(0)=\strains_0$
% 		\Ensure Optimal posture $\pose:[0,L]\to\SE{3}$ 
% 		\State Initialize: decision variable trajectory $\decisionvariables^{(0)}(s)$
% 		\For{$k=0$ to MaxIter}
%     		\State Update state $\pose^{(k)}(s),~\strains^{(k)}(s)$
%     		\Statex \quad\quad by integrating \eqref{eq:pose_evolution}, \eqref{eq:strains_evolution} forwardly.
% 	    	\State Update reduced costate $\internalcouples^{(k)}(s),~\internalforces^{(k)}(s),~\costatestrains^{(k)}(s)$ 
% 	    	\Statex \quad\quad by integrating \eqref{eq:smoothing_problem_reduced_costatepose_evolution}, \eqref{eq:smoothing_problem_reduced_costatestrains_evolution} backwardly
% 	    	\Statex \quad\quad with jump condition \eqref{eq:smoothing_problem_reduced_costate_jump_condition}
% 		    \State Update decision variables pointwisely 
% 		    \Statex \quad\quad from $\decisionvariables^{(k)}(s)$ to $\decisionvariables^{(k+1)}(s)$ by using \eqref{eq:update_law}
% 		\EndFor
% 		\State Output the final posture $\pose$ by integrating \eqref{eq:pose_evolution}
% 		\Statex \quad with final strain trajectory $\strains^{(\text{MaxIter})}(s)$
% 	\end{algorithmic}
% \end{algorithm}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



% =============== Result and Discussion =========================== 
% To demonstrate and evaluate our concept, we conducted series of experiments as the following.
% To prove a physics-informed strain reconstruction, we validated in an arbitrarily generated six strain functions, and we applied our algorithm with restricted number of pose data.
% Next, we collected the kinematic data of the single BR$^2$ with individual actuation mode and computed the posture with the reconstructed strains (Fig.\ref{fig:3}).
% In addition, we cross-validated the accuracy of the tip position by simultaneously measuring the posture using the magnetic sensor.
% Lastly, we introduce serially extended BR$^2$ and cable-driven arm, expected to have complex motions with all modes of strain, to test robustness.


% The result of the synthetic-data study is summarized in Fig.\ref{fig:5}.
% One of the reconstruction result with 5 data points is plotted on the left panel.
% % Discussion statement here
% The center panel shows the overlay of reconstructed strains compared with the ground truth strains.
% The reconstructed modes of strains also match well with the given strain functions.
% The deviation of the strain with respect to the number of data points is shown on the last panel, 
% Six data sets are prepared, each with different number of equispaced pose measurements, based on the synthetic arm.
% We used $\mathcal{L}_2$-error to measure overall %using the mean relative error of strains with respect to the ground truth.
% Error plot implies that the algorithm is able to reconstruct accurate posture with small number of data points.
% Specifically, the reconstructed strains have error less than $1\%$ in both shear and curvature with five data points.


% The experiment is conducted with an initially-straight BR2 going through bending, twisting and mixing motions,
% and the smooth positions and directors are well aligned with the video data (Fig. \ref{fig:3}).
% The corresponding plots for curvature $\kappa_1$ and twist $\kappa_3$ shows that curvature $\kappa_1$ changes in bending motion and twist $\kappa_3$ changes in twisting motion.
% The changes of both curvature $\kappa_1$ and twist $\kappa_3$ are observed in the the mix motion.

% %estimated tip error with respect to ground truth
% To evaluate the tip error, we conduct an experiment with magnetic sensor attached to the tip of the manipulator.
% The error can be calculated between the estimated value and reading from the magnetic sensor.
% In figure ???, we show that the error is within $X\%$.

% For mixed motions in 2 segment manipulator, we conduct the experiments on a serial BR2 and a cable-driven arm.
% BR2 has motions with bending on the upper segment and twisting on the lower segment.
% The cable-driven arm has bending on both segments in two different directions and experiences twisting due to gravity.
% Both manipulators have the smoothing positions and directors well-aligned with the camera tracking result (
% Fig. \ref{fig:4}).
% In addition, the corresponding reconstructed strains at the last frame are shown.


% %Deviation with respect to tracking data number of markers
% To evaluate the estimated error for a middle point, we reduce the number of given data to the smoothing algorithm, and estimate the positions and directors for the missing data points.
% The error can be calculated with the estimated value and the camera tracking value.
% In figure ???, we show that the error is within $X\%$.

% % (3) robustness testing - (1) how many points needed to reconstruct complex arm? (2)(minor)estimated error for the middle points with respect to tracking data,
% % (3)the method can handle noisy data


% %including the number of sampling points needed for reliable reconstruction and the capability to handle noisy data.perform robustness test 

% %Robustness noise
% % To evaluate the robustness of the proposed method, we add noise to the camera tracking data and feed into the smoothing algorithm.
% % The noise is set to be $5\%$ of the original data.
% % The estimated error is the average distance between the prediction and the marker data points.
% % The error is within $X\%$, and indicates the proposed method is relatively robust.

==> IEEEtran/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

